Generation of skill-specific maps from graph world models for robotic systems

With the increase in the availability of Building Information Models (BIM) and (semi-) automatic tools to generate BIM from point clouds, we propose a world model architecture and algorithms to allow the use of the semantic and geometric knowledge encoded within these models to generate maps for robot localization and navigation. When heterogeneous robots are deployed within an environment, maps obtained from classical SLAM approaches might not be shared between all agents within a team of robots, e.g. due to a mismatch in sensor type, or a difference in physical robot dimensions. Our approach extracts the 3D geometry and semantic description of building elements (e.g. material, element type, color) from BIM, and represents this knowledge in a graph. Based on queries on the graph and knowledge of the skills of the robot, we can generate skill-specific maps that can be used during the execution of localization or navigation tasks. The approach is validated with data from complex build environments and integrated into existing navigation frameworks.

==> Chapters/Introduction.tex <==
\section{Introduction}
The large-scale deployment of robotic systems in different sectors such as logistics~\cite{farinelli2017advanced} and agriculture~\cite{fountas2020agricultural} calls for novel approaches for the representation of environmental knowledge shared between several and potentially heterogeneous robots in terms of sensorial and (motion) skills.
Typical requirements posed to large-scale robotic systems relate to their ease of deployment and possibilities for semi-automatic reconfiguration. 
Research shows that both requirements can be addressed by designing knowledge bases shared by the heterogeneous robots which allow information sharing between them as well as the automatic re-configuration of skills and maps (e.g.~\cite{tenorth2017representations, waibel2011roboearth}).
In this paper, we propose a novel approach to designing knowledge bases, in the form of graph world models, that can be shared by heterogeneous robots and from which robot-specific views can be generated. 

The proposed graph world model represents the building elements of an environment with associated semantic properties and geometry. By using the semantics to query the specific building elements and by interpreting the geometry based on the specifics of the robot, we demonstrate that it is possible to automatically generate robot-specific views (e.g. tailored to the type or height of its sensors, or the physical dimensions of the robot itself) in the form of environmental maps which can be integrated in navigation and localization frameworks. 
We particularly focus on ease of deployment addressing the latter from two perspectives: the automatic initialization of the graph world models from Building Information Models (BIM) and the automatic extraction of robot-specific maps from the shared world model.
The graph is initialized by interpreting data from  Building Information Models (BIM) exported in the Industry Foundation Classes (IFC) format~\cite{IFC}. Building on our previous work~\cite{de2021queries, hendrikx2021connecting, pauwels2023live}, the semantics and the geometry of the building elements are extracted and their relations are represented in the topology of an RDF graph. The use of BIM and IFC is relevant to industrial facilities such as warehouses for which these models are normally available and used throughout the design of the logistic process~\cite{he2021bim}. If a BIM model is not available, it is still possible to create one by collecting point-cloud scans of the environment \cite{BOSCHE2010107,BOSCHE2015201}. The point cloud is subsequently segmented into semantic objects of interest, annotated and converted to a BIM model. This is a common procedure in the architectural and infrastructure domain (e.g.,~\cite{soilan20203d, qu2015usage}). Since both initialization paths result in a BIM model, the same algorithm for the construction of the graph world model can be applied. 
Second, we provide methods to generate skill-specific environmental representations derived from the graph world model focusing on robots using 2D LIDAR for navigation and localization. We show that the map generation process can be tailored to the specific skills and physical properties of the robot by only representing those elements in the world model which are selected based on the properties of the specific skill and robot.
The concept presented in the paper is displayed in Fig.~\ref{fig:concept}.
The methods are validated considering graph world models of a large university building as well as a simple lab environment.
We demonstrate the feasibility of integrating the generated maps into existing navigation algorithms by enabling a small robot to autonomously navigate a lab environment for which a graph world model is available. 
The remainder of the paper is organized as follows. Section~\ref{sec:rel_work} positions this work with respect to the state-of-the-art. Section~\ref{sec:graphWorldModel} provides a formal definition of the graph's concepts and topology and introduces methods for its automatic initialization from BIM/IFC models. Section~\ref{sec:map_generation} introduces the queries and the methods to extract the geometry of identified semantic elements and to create navigation and localization maps tailored to the skills of the robot requesting them. The results demonstrate the potential for the integration of the generated maps into existing navigation frameworks. Finally, Section~\ref{sec:DiscAndConcl} provides an interpretation of the results discussing the potential and limitations of the presented methods and outlines future research directions.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{Figures/Architecture.png}
  \caption{Conceptual architecture. Blue: provided input. Green: novel algorithms. Orange: algorithm's output. }
  \label{fig:concept}
\end{figure}

==> Figures/GraphDerivation.tex <==
\begin{tikzpicture}[
    every node/.style={font=\normalsize}
]

\def\scale{2}
\def\length{\scale*4}
\def\width{\scale*4}
\def\doorwidth{\scale*0.65}
\def\divwallheight{0.5*\length}
\def\interfaceoffset{\scale*0.1}
\def\shorten_interfaceoffset{1.5*\interfaceoffset}

\coordinate (leftbottom) at (0,0) {};
\coordinate (righttop) at (\width, \length) {};

\coordinate(centertop) at (\width/2, \length){};
\coordinate(centertop_offset) at (\width/2, \length-\doorwidth){};

\coordinate(centerbottom) at (\width/2, 0){};
\coordinate(centerbottom_offset) at (\width/2, \doorwidth){};
\coordinate(div_wall_left) at (0, \divwallheight){};
\coordinate(div_wall_right) at (\width/2, \divwallheight){};

\draw (leftbottom) rectangle (righttop);	
\draw [draw=none] (leftbottom) rectangle (0.5*\width, 0.5*\length) node[midway, font=\normalsize] {S1};
\draw [draw=none] (div_wall_left) rectangle (centertop) node[midway, font=\normalsize] {S2};	
\draw [draw=none] (righttop) rectangle (centerbottom) node[midway, font=\normalsize] {S3};	

\node[left] at ($(leftbottom)!0.25!(leftbottom |- righttop)$) {W1.1};
\node[left] at ($(leftbottom)!0.75!(leftbottom |- righttop)$) {W2.1};
\node[below] at ($(leftbottom)!0.5!(leftbottom -| righttop)$) {W1.3};
\node[above] at ($(righttop)!0.5!(righttop -| leftbottom)$) {W3.1};
\node[right] at ($(righttop)!0.5!(righttop |- leftbottom)$) {W3.2};


\draw (centerbottom_offset) --  (centertop_offset) node[midway, below, sloped] {W3.2};

\draw (div_wall_left) -- (div_wall_right) node[midway, above] {W1.2};

\draw [red] (div_wall_left) ++(\shorten_interfaceoffset, -\interfaceoffset) -- ($(div_wall_right) + (-\shorten_interfaceoffset,-\interfaceoffset)$) node[midway, below, sloped] {IF1.2};
\draw [red] (leftbottom) ++(\interfaceoffset,\shorten_interfaceoffset) -- ($(div_wall_left) + (\interfaceoffset,-\shorten_interfaceoffset)$) node[midway, below, sloped] {IF1.1};
\draw [red] (leftbottom) ++(\shorten_interfaceoffset,\interfaceoffset) -- ($(centerbottom) + (-\shorten_interfaceoffset,\interfaceoffset)$) node[midway, above, sloped] {IF1.3};
\draw [red] (div_wall_right) ++(-\interfaceoffset,-\shorten_interfaceoffset) -- ($(centerbottom_offset) + (-\interfaceoffset,\shorten_interfaceoffset)$) node[midway, below, sloped] {IF1.4};

\draw(centertop_offset) -- ++(-\doorwidth, 0);
\draw [red](centertop_offset)  ++(-\shorten_interfaceoffset, \interfaceoffset)  -- ++(-\doorwidth + 2*\shorten_interfaceoffset, 0 ) node[midway, above, sloped] {IF3.1};
\draw [red](centertop_offset)  ++(-\shorten_interfaceoffset, -\interfaceoffset)  -- ++(-\doorwidth + 2*\shorten_interfaceoffset, 0)node[midway, below, sloped] {IF2.1};

\draw(centerbottom_offset) -- ++(-\doorwidth, 0);
\draw [red](centerbottom_offset)  ++(-\shorten_interfaceoffset, \interfaceoffset)  -- ++(-\doorwidth + 2*\shorten_interfaceoffset, 0)  node[midway, above, sloped] {IF1.5};
\draw [red](centerbottom_offset)  ++(-\shorten_interfaceoffset, -\interfaceoffset)  -- ++(-\doorwidth + 2*\shorten_interfaceoffset, 0)  node[midway, below, sloped] {IF3.2};


\draw [red] (centerbottom) ++(\shorten_interfaceoffset,\interfaceoffset) -- ($(\width,0) + (-\shorten_interfaceoffset,\interfaceoffset)$) node[midway, above, sloped] {IF3.3};
\draw [red] (righttop) ++(-\interfaceoffset,-\shorten_interfaceoffset) -- ($(\width,0) + (-\interfaceoffset,\shorten_interfaceoffset)$) node[midway, below, sloped] {IF3.4};
\draw [red] (centertop) ++(\shorten_interfaceoffset, -\interfaceoffset) -- ($(righttop) + (-\shorten_interfaceoffset,-\interfaceoffset)$) node[midway, below, sloped] {IF3.5};
\draw [red] (centerbottom_offset) ++(\interfaceoffset,\shorten_interfaceoffset) -- ($(centertop_offset) + (\interfaceoffset,-\shorten_interfaceoffset)$) node[pos=0.75, below, sloped] {IF3.6};

\draw [red] (div_wall_left) ++(\interfaceoffset,\shorten_interfaceoffset) -- ($(0,\length) + (\interfaceoffset,-\shorten_interfaceoffset)$) node[midway, below, sloped] {IF2.2};
\draw [red] (0, \length) ++(\shorten_interfaceoffset, -\interfaceoffset) -- ($(centertop) + (-\shorten_interfaceoffset,-\interfaceoffset)$) node[midway, below, sloped] {IF2.3};
\draw [red] (centertop_offset) ++(-\interfaceoffset,-\shorten_interfaceoffset) -- ($(div_wall_right) + (-\interfaceoffset,\shorten_interfaceoffset)$) node[midway, below, sloped] {IF2.4};
\draw [red] (div_wall_left) ++(\shorten_interfaceoffset, \interfaceoffset) -- ($(div_wall_right) + (-\shorten_interfaceoffset,\interfaceoffset)$) node[pos=0.75, above, sloped] {IF2.5};



\draw [] (centertop_offset) ++(-\doorwidth, 0) arc (180:90:\doorwidth);
\draw [] (centerbottom_offset) ++(-\doorwidth, 0) arc (180:270:\doorwidth);
\end{tikzpicture}

==> Figures/GraphDerivation2.tex <==
\begin{tikzpicture}[
  node distance =2.5cm, % Adjust this value for your desired spacing
  node/.style = {circle, draw, minimum size=1.25cm}
]
  % Create nodes
  \node (S1)[node] {S1};
  \node (IF12) [node, above of=S1] {IF1.2};
  \node (W12) [node, above of=IF12] {W1.2};
  \node (IF25) [node, above of=W12] {IF2.5};
  \node(S2)[node, left of=IF25]{S2};
  
  \node (IF11) [node, left of=IF12] {IF1.1};
  \node (W11) [node, above of=IF11] {W1.1};
  
  \node(IF15)[node, below of=S1]{IF1.5};
  \node(IF14)[node, right of=S1]{IF1.4};
  \node(D11)[node, right of=IF15]{D1.1};
  \node(W32)[node, above of=IF14]{W3.2};
  \node(IF36)[node, right of=W32]{IF3.6};
  \node(IF32)[node, right of=D11]{IF3.2};
  
  \node (IF13) [node, left of=IF15] {IF1.3};
  \node (W13) [node, above of=IF13] {W1.3};

  \node(S3)[node, right of=IF14]{S3};
  
\draw (S1) -- (IF11);
\draw (W11) -- (IF11);
\draw (S1) -- (IF12);
\draw (W12) -- (IF12);
\draw (S1) -- (IF13);
\draw (W13) -- (IF13);
\draw(W12) -- (IF25);
\draw(IF25)--(S2);
\draw(S1)--(IF14);
\draw(S1)--(IF15);
\draw(IF15)--(D11);
\draw(IF14)--(W32);
\draw(IF36)--(W32);
\draw(IF32)--(D11);
\draw(IF32)--(S3);
\draw(IF36)--(S3);

\end{tikzpicture}

==> Figures/GraphRoom.tex <==
\begin{tikzpicture}[align=center,node distance=2.25cm]

\definecolor{myred}{rgb}{0.906,0.298,0.235}
\definecolor{myblue}{rgb}{0.204, 0.596, 0.859}
\definecolor{myyellow}{rgb}{0.992,0.796,0.431}
\definecolor{mygray}{rgb}{0.698, 0.745, 0.765}
\definecolor{mygreen}{rgb}{0.152, 0.682, 0.376}
\definecolor{mypurple}{rgb}{0.698, 0.745, 0.765}
\definecolor{mybrown}{rgb}{0.882, 0.439, 0.333}


%% Space 1
\node [circle, draw] (F1) at (0, 0) {\normalsize Floor\_1};
\node [circle, draw, above left = of F1] (W1) {\normalsize Wall\_1};
\node [circle, draw, above right = of F1] (W3) {\normalsize Wall\_3};
\node [circle, draw, right = of F1] (W2) {\normalsize Wall\_2};
\node [circle, draw, left = of F1] (W4) {\normalsize Wall\_4};
\node [circle, draw, below left = of F1] (C1) {\normalsize Chair};
\node [circle, draw, below right = of F1] (T1) {\normalsize Table};


\draw [-latex]  (W1) edge node [anchor = south west, left] { \normalsize is adjacent to} (F1);
\draw [-latex]  (W3) edge node [anchor = north west, right] { \normalsize is adjacent to} (F1);
\draw [-latex]  (W4) edge node [anchor = north west, above] { \normalsize is adjacent to} (F1);
\draw [-latex]  (W2) edge node [anchor = north west, above] { \normalsize is adjacent to} (F1);

\node [circle, draw, left = of W1] (D1) {\small Door};
\node [circle, draw, right = of W3] (Wi1) {\small Window};

\draw [-latex]  (D1) edge node [anchor = south west, above] { \normalsize is contained in} (W1);
\draw [-latex]  (Wi1) edge node [anchor = north west, above]{ \normalsize is contained in} (W3);
\draw [-latex]  (C1) edge node [anchor = south west, left] { \normalsize is contained in} (F1);
\draw [-latex]  (T1) edge node [anchor = north west, right] { \normalsize is contained in} (F1);


\end{tikzpicture}

==> Figures/concept.tex <==
\begin{tikzpicture}
  \node [draw, cylinder, shape aspect=0.7, minimum height=4.5cm, minimum width=3cm, shape border rotate=90] (database) {Graph World Model};
  \node [draw, anchor=west, minimum width=2.5cm, minimum height=1.5cm] (rect1) at (-6,2) {BIM};
  \node [draw, anchor=west, minimum width=2.5cm, minimum height=1.5cm] (rect2) at (-6,-1) {Point Cloud};

  % Arrows from rectangles to the cylinder with LaTeX arrowheads, text "initialize," and larger size, sloped along the arrow
  \draw[-latex, line width=2pt] (rect1.east) -- (database.west) node[midway, above, sloped] {initialize};
  \draw[-latex, line width=2pt] (rect2.east) -- (database.west) node[midway, above, sloped] {initialize};

  % Box to the right of the cylinder with text, aligned with the top of the database
  \node [draw, yshift = 1.5 cm, right=1.5 cm of database.east, anchor=west, minimum width=7cm, minimum height=2cm] (box) {Skill-specific map generator};

  % Three boxes centered underneath the "Skill-specific map generator" box
  \node [draw, below=2 cm of box.south west, anchor=west, minimum width=2cm, minimum height=1cm] (box1) {Robot A};
  \node [draw, right=1.0cm of box1.east, minimum width=2cm, minimum height=1cm] (box2) {Robot B};
  \node [draw, right=0.5cm of box2.east, minimum width=2cm, minimum height=1cm] (box3) {Robot C};

  \draw[-latex, line width=2pt] ([xshift=-2.25cm] box.south) -- ([xshift=0.25cm] box1.north) node[pos=0.5, left, xshift=-0.5 cm, align=center] {Robot \\ Skill \\ Properties};
  \draw[-latex, line width=2pt] ([xshift=-0.25cm] box1.north) -- ([xshift=-2.75cm] box.south) node[pos=0.5, , xshift=0.5 cm ,right,  align=center] {Generated \\ Specific \\ Map};
   
   \draw[-latex, line width=2pt] ([xshift=0.25cm] box.south) -- ([xshift=-0.25cm] box2.north);
   \draw[-latex, line width=2pt] ([xshift=0.25cm] box2.north) -- ([xshift=0.75cm] box.south);
   
   \draw[-latex, line width=2pt] ([xshift=3.25cm] box.south) -- ([xshift=0.25cm] box3.north);
   \draw[-latex, line width=2pt] ([xshift=-0.25cm] box3.north) -- ([xshift=2.75cm] box.south); 
  
 \draw[-latex, line width=2pt] ([yshift=1.5cm] database.east) -- (box.west);
\end{tikzpicture}
